Optimal Heaviest Induced Ancestors

We revisit the Heaviest Induced Ancestors (HIA) problem that was introduced by Gagie, Gawrychowski, and Nekrich [CCCG 2013] and has a number of applications in string algorithms. Let $T_1$ and $T_2$ be two rooted trees whose nodes have weights that are increasing in all root-to-leaf paths, and labels on the leaves, such that no two leaves of a tree have the same label. A pair of nodes $(u, v)\in T_1 \times T_2$ is \emph{induced} if and only if there is a label shared by leaf-descendants of $u$ and $v$. In an HIA query, given nodes $x \in T_1$ and $y \in T_2$, the goal is to find an induced pair of nodes $(u, v)$ of the maximum total weight such that $u$ is an ancestor of~$x$ and $v$ is an ancestor of $y$. Let $n$ be the upper bound on the sizes of the two trees. It is known that no data structure of size $\tilde{\mathcal{O}}(n)$ can answer HIA queries in $o(\log n / \log \log n)$ time [Charalampopoulos, Gawrychowski, Pokorski; ICALP 2020]. This (unconditional) lower bound is a $\operatorname{polyloglog} n$ factor away from the query time of the fastest $\tilde{\mathcal{O}}(n)$-size data structure known to date for the HIA problem [Abedin, Hooshmand, Ganguly, Thankachan; Algorithmica 2022]. In this work, we resolve the query-time complexity of the HIA problem for the near-linear space regime by presenting a data structure that can be built in $\tilde{\mathcal{O}}(n)$ time and answers HIA queries in $\mathcal{O}(\log n/\log\log n)$ time. As a direct corollary, we obtain an $\tilde{\mathcal{O}}(n)$-size data structure that maintains the LCS of a static string and a dynamic string, both of length at most $n$, in time optimal for this space regime. The main ingredients of our approach are fractional cascading and the utilization of an $\mathcal{O}(\log n/ \log\log n)$-depth tree decomposition.

==> cases.tex <==
\begin{tikzpicture}

\node[fill,circle,scale=0.4] (A) at (0,0) {};
\node[fill,circle,scale=0.4] (C) at (0,-1) {};
\node (C-desc) at (0.2,-1) {$x$};
\node[fill,circle,scale=0.4] (F) at (0,-2.5) {};
\node (F-desc) at (0.2,-2.5) {$w$};
\draw (F) -- (-1,-3.5) -- (-1.7,-4.8) -- (-0.3,-4.8) -- (-1,-3.5);
\node[fill,circle,scale=0.4] (X) at (-1.3,-4.8) {};
\node (X-desc) at (-1.1,-4.6) {$\ell$};
\node[fill,circle,scale=0.4] (G) at (0,-3) {};

\path[draw,ultra thick] (A) -- (C) -- (F) -- (G);
\path[draw] (0,0.5) -- (-1.9,-3.2) -- (1.9,-3.2) -- (0,0.5);

\end{tikzpicture}

\hspace{3cm}

\begin{tikzpicture}

\node[fill,circle,scale=0.4] (A) at (0,0) {};
\node[fill,circle,scale=0.4] (B) at (0,-0.5) {};
\node (B-desc) at (0.2,-0.5) {$w$};
\node[fill,circle,scale=0.4] (E) at (0,-2) {};
\node (E-desc) at (0.2,-2) {$x$};
\draw (B) -- (-3,-1.5) -- (-3.7,-2.8) -- (-2.3,-2.8) -- (-3,-1.5);
\node[fill,circle,scale=0.4] (X) at (-3.3,-2.8) {};
\node (X-desc) at (-3.1,-2.6) {$\ell$};
\node[fill,circle,scale=0.4] (G) at (0,-3) {};

\path[draw] (0,0.5) -- (-2.2,-3.2) -- (2.2,-3.2) -- (0,0.5);
\path[draw,ultra thick] (A) -- (B) -- (E) -- (G);

\end{tikzpicture}

\hspace{3cm}

\begin{tikzpicture}

\node[fill,circle,scale=0.4] (AA) at (1,-1) {};
\node[fill,circle,scale=0.4] (CC) at (1,-2) {};
\node[fill,circle,scale=0.4] (EE) at (1,-3) {};
\node (C-desc) at (1.2,-2) {$x$};
\node[fill,circle,scale=0.4] (A) at (0,0) {};
\node[fill,circle,scale=0.4] (G) at (0,0.8) {};
\node (G-desc) at (0.2,0.8) {$w$};
\node[fill,circle,scale=0.4] (I) at (0,1.6) {};
\draw (G) -- (-3,-0.2) -- (-3.7,-1.5) -- (-2.3,-1.5) -- (-3,-0.2);
\node[fill,circle,scale=0.4] (X) at (-3.3,-1.5) {};
\node (X-desc) at (-3.1,-1.3) {$\ell$};


\path[draw,ultra thick] (AA) -- (CC) -- (EE);
\path[draw,ultra thick] (I) -- (G) -- (A);
\path[draw,dotted] (A) .. controls +(0.5,0.3) and +(-0.5,-0.3) .. (AA);
\path[draw] (0,2.1) -- (-2.5,-3.2) -- (2.5,-3.2) -- (0,2.1);

\end{tikzpicture}

